Extensible Data Skipping

Data skipping reduces I/O for SQL queries by skipping over irrelevant data objects (files) based on their metadata. We extend this notion by allowing developers to define their own data skipping metadata types and indexes using a flexible API. Our framework is the first to natively support data skipping for arbitrary data types (e.g. geospatial, logs) and queries with User Defined Functions (UDFs). We integrated our framework with Apache Spark and it is now deployed across multiple products/services at IBM. We present our extensible data skipping APIs, discuss index design, and implement various metadata indexes, requiring only around 30 lines of additional code per index. In particular we implement data skipping for a third party library with geospatial UDFs and demonstrate speedups of two orders of magnitude. Our centralized metadata approach provides a x3.6 speed up even when compared to queries which are rewritten to exploit Parquet min/max metadata. We demonstrate that extensible data skipping is applicable to broad class of applications, where user defined indexes achieve significant speedups and cost savings with very low development cost.

==> background.tex <==
\section{Background}
Today?s   best   practices   to   deploy   and   manage   cloud   compute   and   storage   services   independently leaves us with a problem: potentially huge datasets need to be shipped from the storage service to the compute service to analyse data. If this data needs to be sent  across  the  WAN  then  this  is  even  more  critical.  Therefore,  it  becomes  of  ultimate  importance  to  minimize  the  amount  of  data  sent  across  the  network,  since  this  is  the  key  factor  affecting  cost  and  performance  in  this  context. Many  cloud-based  SQL  services,  for  example  Amazon  Athena,  bill  users  according  to  the  amount  of  data  scanned  in  object  storage, outlining the importance of this metric. 

There are currently three main approaches to limit the number of bytes sent from the storage to Spark. (Note we focus on object storage although this can also be applied more broadly). The  first  is  to  use  specialized  column  based  formats  such  as  Parquet  and  ORC.  These formats provide column wise compression, which significantly reduces the number of bytes to  be  sent.  They  also  support  column  pruning,  so  that  only  columns  requested  by  a  query need to be sent to Spark. Finally, they sometimes support specialized metadata which can be used to filter columns following query predicates.  Parquet can provide more than an order magnitude performance improvement over other formats such as csv.

The  second  approach  is  to  use  Hive  style  partitioning  to  name  the  objects  using  a  certain  convention. In this case, information about object contents is encoded into object names. For example,  if  we  partition  per  a date  column  then  each  object  will  contain  data  records  with  the  same  date,  and  the  date  is  encoded  in  the  object  name.  Spark  SQL  understands  this  convention  and  can  filter  the  set  of  objects  retrieved  when  query  predicates  apply  to  partitioning columns. This can significantly reduce the number of objects sent to Spark and the number of bytes shipped .    The third approach is called Data Skipping and it can complement the first two approaches. This approach utilizes metadata to track information about objects and their dataset columns which can then be used for data skipping i.e. to show that an object is not relevant to a query and therefore does not need to be accessed from storage or sent on the network from object storage to Spark. IBM Research implemented Data Skipping technology in the context of the IOStack H2020 project45.  To make it efficient, we indexed the metadata, so that during query execution, can quickly filter out irrelevant objects from the list of objects to be accessed by the query. Note that this technique applies to all data formats, and avoids touching irrelevant objects altogether (see our presentation46at the Spark Summit, where Databricks announced Data Skipping support in their platform.

\subsection{Data Skipping Indexes}
Data skipping is a technique used for big data analytics on tabular data (comprising multiple rows) whereby summary metadata is stored for row subsets. This summary metadata can be used to determine that a row subset is irrelevant to a query (e.g. in SQL) and therefore can be skipped during query processing. This results in significant performance improvements and cost reductions.

To date, data skipping is typically stored per column and works when:
- the column is numeric e.g. integer, float, and the query predicate is one of <, <=, >, >=, = 
In this case the summary metadata used is the minimum and maximum values for a column
- the column is numeric or string and the query predicate is one of =, IN
In this case the summary metadata used is a list of values or a bloom filter.


\subsection{Data Skipping versus Data Layout}

\subsection{Formats}

\subsection{Object Storage}

\subsection{Apache Spark}


